LearnMate: Enhancing Online Education with LLM-Powered Personalized Learning Plans and Support

With the increasing prevalence of online learning, adapting education to diverse learner needs remains a persistent challenge. Recent advancements in artificial intelligence (AI), particularly large language models (LLMs), promise powerful tools and capabilities to enhance personalized learning in online educational environments. In this work, we explore how LLMs can improve personalized learning experiences by catering to individual user needs toward enhancing the overall quality of online education. We designed personalization guidelines based on the growing literature on personalized learning to ground LLMs in generating tailored learning plans. To operationalize these guidelines, we implemented LearnMate, an LLM-based system that generates personalized learning plans and provides users with real-time learning support. We discuss the implications and future directions of this work, aiming to move beyond the traditional one-size-fits-all approach by integrating LLM-based personalized support into online learning environments.

==> related_llm.tex <==

% \subsection{personalization/adaptation efforts in ml}


\subsection{Personalization and Adaptation in the Era of LLMs}

In the era dominated by LLMs, encompassing commercial LLMs (\eg GPT-4~\cite{gpt-4}, Gemini families~\cite{geminiteam2023gemini}, and Claude~\cite{claude}) and ``open source'' LLMs (\eg LLaMA~\cite{touvron2023llama}, Grok~\cite{grok}, and Mistral~\cite{jiang2023mistral}), we have witnessed the remarkable capabilities of these models in generating human-like text and understanding contextual cues.
Nonetheless, just having an LLM generate answers based on its pre-training has a clear limitation: although the most-capable LLMs have been trained on large swaths of the internet, they would not have seen documents generated past a specific training cutoff date, and certainly could not have seen personal/enterprise documents, documents behind paywalls, data in databases, and so on.
To overcome such limitation, there are two common approaches for incorporating domain-specific information into LLMs for their personalized usage: fine-tuning and Retrieval Augmented Generation (RAG).
% has fostered a new level of personalization and adaptation.

% LLMs have been extensively used for personalization, thanks to their ability to model user interactions and generate responses that align with user's needs and preferences. 
% For instance, GPT-2 was used by~\citet{radford2019language} to generate personalized responses in dialogue systems, thereby enhancing user engagement. Similarly,~\citet{zhang2020dialogpt} employed BERT for personalizing chatbots, making responses more contextually relevant and personalized, and consequently improving user experience.

% Personalization and adaptation using LLMs have commonly relied on two key approaches: fine-tuning and Reinforcement Learning from Human Feedback (RLHF). 
Fine-tuning involves adapting the pre-trained LLM to a specific task or user data by continuing the training process, thereby enabling the models to learn the nuances and requirements of the target domain~\cite{houlsby2019parameter, zhang2020dialogpt}. 
However, the fine-tuning approach requires substantial computational resources and expertise, as well as full white-box access to the model's internals, which is not a realistic assumption since LLM model weights are often protected by the model provider's intellectual property laws.
Moreover, it risks catastrophic forgetting, where the model loses its ability to perform tasks it was previously good at, and the severity of forgetting increases as the model scale increases~\cite{luo2023empirical}. 
Other than adaptation to target task, Reinforcement Learning from Human Feedback (RLHF) can help align LLMs with user preferences~\cite{bai2022rlhf}.
RLHF involves the additional steps of training a Reward Model with preference data, which consists of prompts and multiple candidate outputs ranked by human evaluators. Then it uses the reward model to fine-tune the LLM through reinforcement learning 
to align the LLM's behavior with human preferences and values defined via reward modeling.
% This approach, used by Bahdanau et al., (2018) for training a dialogue system, allows for continuous model improvement. 
% Bahdanau, D., Chattopadhyay, A., Serdyuk, D., Wallach, H., & Courville, A. (2018). An actor-critic algorithm for sequence prediction. In International Conference on Learning Representations (ICLR).
Yet, the performance of RLHF largely depends on reward modeling and the quality and quantity of human feedback, which can be challenging to obtain, and it shares the computational expense and complexity of the fine-tuning approach. This makes fine-tuning and RLHF-based approaches less accessible to individual users who may want to leverage state-of-the-art off-the-shelf LLMs like GPT-4, OpenAI's Codex, or Google's LaMDA for personal use.

% A more recent alternative to these methods is the Retrieval-Augmented Generation (RAG) approach. Just having an LLM generate answers based on its pre-taining has two limitations: (a) although the most-capable LLMs have been trained on large swaths of the internet, they would not have \textit{seen} documents generated past a specific training cutoff date, and certainly could not have seen personal/enterprise documents, documents behind paywalls, data in databases, and so on. (b) Even if an LLM generates an answer, there is no way to verify the validity of the answer as it does not include a source citation. 
On the other hand, RAG provides more flexibility to adapt to changing data without retraining the entire model, by only requiring black-box access to the model (\ie via API calls).
It allows the model to leverage knowledge sources (\eg specific documents on personal information or instructions, or an external database) not present in the original training data of the deployed LLM. 
It retrieves relevant information from the external knowledge and uses it to guide the response generation by augmenting the user input prompt~\cite{lewis2020retrieval}.  
% The RAG approach addresses both of these limitations by retrieving relevant information from a knowledge source (\eg specific documents or an external database) and using it to guide the response generation~\cite{lewis2020retrieval}.
% RAG combines the strengths of powerful pre-trained models and information retrieval to generate responses~\cite{lewis2020retrieval}. 
% This method is computationally efficient and versatile, and more importantly,
% RAG can be used with just API access to the LLMs, making it a more accessible approach for individuals wanting to make adaptive use of any black-box LLMs for personal use cases.
This method is not only computationally efficient and versatile, compared to fine-tuning or RLHF approaches that necessitate additional training, but is also accessible to individuals who wish to adaptively use any black-box LLMs for personal use cases.
% , as it only requires API access to the LLMs.
More importantly, it is possible with RAG to verify the validity of the generated answer by including a source citation. 


There have been a few recent attempts to explore the use of RAG in the context of personalized dialogue generation, such as persona profiles and distinctive authorial nuances~\cite{rag-style, lapdog}. 
% \citet{rag-style} proposes a style-based RAG approach, where the style embeddings are used to capture distinctive authorial nuances for the purpose of personalizing LLMs. 
However, the focus of personalization in our work rather lies in handling conflicting multiple user requests and supporting decision-making adapted to individual preferences and instructions.
To the best of our knowledge, our work is the first to propose a RAG approach with usability for multi-user adaptive personalization.
Moreover, we explore the potential of multi-agent collaboration to address complex personalization requests, in contrast to the monolithic agent-based approaches found in most prior works on RAG-based personalization.
% In conclusion, the era of LLMs has brought significant advancements and opportunities in personalization and adaptation. Despite the challenges, with the right strategies and methodologies such as RAG, these models can offer rich, engaging, and personalized user experiences.

